Increasing Depth of Neural Networks for Life-long Learning

Purpose: We propose a novel method for continual learning based on the increasing depth of neural networks. This work explores whether extending neural network depth may be beneficial in a life-long learning setting. Methods: We propose a novel approach based on adding new layers on top of existing ones to enable the forward transfer of knowledge and adapting previously learned representations. We employ a method of determining the most similar tasks for selecting the best location in our network to add new nodes with trainable parameters. This approach allows for creating a tree-like model, where each node is a set of neural network parameters dedicated to a specific task. The Progressive Neural Network concept inspires the proposed method. Therefore, it benefits from dynamic changes in network structure. However, Progressive Neural Network allocates a lot of memory for the whole network structure during the learning process. The proposed method alleviates this by adding only part of a network for a new task and utilizing a subset of previously trained weights. At the same time, we may retain the benefit of PNN, such as no forgetting guaranteed by design, without needing a memory buffer. Results: Experiments on Split CIFAR and Split Tiny ImageNet show that the proposed algorithm is on par with other continual learning methods. In a more challenging setup with a single computer vision dataset as a separate task, our method outperforms Experience Replay. Conclusion: It is compatible with commonly used computer vision architectures and does not require a custom network structure. As an adaptation to changing data distribution is made by expanding the architecture, there is no need to utilize a rehearsal buffer. For this reason, our method could be used for sensitive applications where data privacy must be considered.

==> images/structure_schema.tex <==
\begin{tikzpicture}[node distance=0.6cm, auto,
    squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick},
    trapezenode/.style={trapezium, trapezium angle=75, very thick},
    imagenode/.style={trapezium, trapezium left angle=60, trapezium right angle=-60, minimum width=1.6cm, minimum height=0.5cm, ultra thin, fill=white!5, draw}
    ]
    %Nodes
    % NETWORK A (One task)
    % common backbone
    \node[trapezenode, draw=red!60, fill=red!5, minimum width=9mm] (conv_1_A) {};
    \node[squarednode, draw=red!60, fill=red!5, minimum width=6mm, minimum height=10mm] [above=0.1cm of conv_1_A] (conv_2_A) {};
    \node[trapezenode, draw=red!60, fill=red!5, minimum width=6mm] [above=0.1cm of conv_2_A] (conv_3_A) {};
    % task 1 node
    \node[squarednode, draw=blue!60, fill=blue!5, minimum width=4mm, minimum height=12mm] [above=0.2cm of conv_3_A] (conv_4_A) {};
    \node[trapezenode, draw=green!60, fill=green!5, minimum width=4mm] [above=0.2cm of conv_4_A] (conv_5_A) {};
    \node[squarednode, draw=green!60, fill=green!5, minimum width=2.5mm, minimum height=15mm] [above=0.1cm of conv_5_A] (conv_6_A) {};
    \node[squarednode, draw=green!60, fill=green!5] [above=0.1cm of conv_6_A] (conv_7_A) {};
    
    % COMMON BACKBONE LABEL
    \node[] [left=0.75cm of conv_2_A, align=left] (backbone_label) {common\\backbone};
    
    % SINGLE NODE STRUCTURE
    \node[] [below=0.001cm of conv_4_A] (anchor) {};
    \node[] [left=0.8cm of anchor] (lower_left) {};
    \node[] [right=0.8cm of anchor] (lower_right) {};
    \node[] [above=3.8cm of lower_left] (upper_left) {};
    \node[] [above=3.8cm of lower_right] (upper_right) {};
    % \node[] [above=3.9cm of anchor] (node_label) {single node structure};
    \node[] [left=1.4cm of conv_5_A, align=left] (node_label) {single\\node};
    % \node[] [left=1.5cm of lower_left] (margin) {};
    
    % NETWORK B (Two tasks)
    % common backbone
    \node[trapezenode, draw=red!60, fill=red!5, minimum width=9mm] (conv_1_B) [right=3.5cm of conv_1_A] {};
    \node[squarednode, draw=red!60, fill=red!5, minimum width=6mm, minimum height=10mm] [above=0.1cm of conv_1_B] (conv_2_B) {};
    \node[trapezenode, draw=red!60, fill=red!5, minimum width=6mm] [above=0.1cm of conv_2_B] (conv_3_B) {};
    % task 1 node
    \node[squarednode, draw=blue!60, fill=blue!5, minimum width=4mm, minimum height=12mm] [above=0.2cm of conv_3_B] (conv_4_B) {};
    \node[trapezenode, draw=green!60, fill=green!5, minimum width=4mm] [above left=of conv_4_B] (conv_5_B) {};
    \node[squarednode, draw=green!60, fill=green!5, minimum width=2.5mm, minimum height=15mm] [above=0.1cm of conv_5_B] (conv_6_B) {};
    \node[squarednode, draw=green!60, fill=green!5] [above=0.1cm of conv_6_B] (conv_7_B) {};
    % task 2 node
    \node[squarednode, draw=blue!60, fill=blue!5, minimum width=4mm, minimum height=12mm] [above right=of conv_4_B] (conv_8_B) {};
    \node[trapezenode, draw=green!60, fill=green!5, minimum width=4mm] [above=0.2cm of conv_8_B] (conv_9_B) {};
    \node[squarednode, draw=green!60, fill=green!5, minimum width=2.5mm, minimum height=15mm] [above=0.1cm of conv_9_B] (conv_10_B) {};
    \node[squarednode, draw=green!60, fill=green!5] [above=0.1cm of conv_10_B] (conv_11_B) {};
    
    % NETWORK C (Three tasks)
    % common backbone
    \node[trapezenode, draw=red!60, fill=red!5, minimum width=9mm] (conv_1_C) [right=4.5cm of conv_1_B] {};
    \node[squarednode, draw=red!60, fill=red!5, minimum width=6mm, minimum height=10mm] [above=0.1cm of conv_1_C] (conv_2_C) {};
    \node[trapezenode, draw=red!60, fill=red!5, minimum width=6mm] [above=0.1cm of conv_2_C] (conv_3_C) {};
    % task 1 node
    \node[squarednode, draw=blue!60, fill=blue!5, minimum width=4mm, minimum height=12mm] [above left=of conv_3_C] (conv_4_C) {};
    \node[trapezenode, draw=green!60, fill=green!5, minimum width=4mm] [above left=of conv_4_C] (conv_5_C) {};
    \node[squarednode, draw=green!60, fill=green!5, minimum width=2.5mm, minimum height=15mm] [above=0.1cm of conv_5_C] (conv_6_C) {};
    \node[squarednode, draw=green!60, fill=green!5] [above=0.1cm of conv_6_C] (conv_7_C) {};
    % task 2 node
    \node[squarednode, draw=blue!60, fill=blue!5, minimum width=4mm, minimum height=12mm] [above right=of conv_4_C] (conv_8_C) {};
    \node[trapezenode, draw=green!60, fill=green!5, minimum width=4mm] [above=0.2cm of conv_8_C] (conv_9_C) {};
    \node[squarednode, draw=green!60, fill=green!5, minimum width=2.5mm, minimum height=15mm] [above=0.1cm of conv_9_C] (conv_10_C) {};
    \node[squarednode, draw=green!60, fill=green!5] [above=0.1cm of conv_10_C] (conv_11_C) {};
    % task 3 node
    \node[squarednode, draw=blue!60, fill=blue!5, minimum width=4mm, minimum height=12mm] [above right=of conv_3_C] (conv_12_C) {};
    \node[trapezenode, draw=green!60, fill=green!5, minimum width=4mm] [above=0.2cm of conv_12_C] (conv_13_C) {};
    \node[squarednode, draw=green!60, fill=green!5, minimum width=2.5mm, minimum height=15mm] [above=0.1cm of conv_13_C] (conv_14_C) {};
    \node[squarednode, draw=green!60, fill=green!5] [above=0.1cm of conv_14_C] (conv_15_C) {};
    
    % TASK ANNOTATIONS
    \node[] [above=6.3cm of conv_3_A] (task_1) {Task 1};
    \node[] [above=6.3cm of conv_3_B] (task_2) {Task 2};
    \node[] [above=6.3cm of conv_3_C] (task_3) {Task 3};
    \node (task_1_2_upper) at ($(task_1)!0.5!(task_2)$) {};
    \node (task_1_2_lower) [below=10cm of task_1_2_upper] {};
    \draw[dotted] (task_1_2_upper) -- (task_1_2_lower);
    \node (task_2_3_upper) at ($(task_2)!0.5!(task_3)$) {};
    \node (task_2_3_lower) [below=10cm of task_2_3_upper] {};
    \draw[dotted] (task_2_3_upper) -- (task_2_3_lower);
    
    % LEGEND
    \node[draw=red!60, fill=red!5] [left=11.7cm of conv_11_C] (red) {};
    \node [right=0.1cm of red, font=\fontsize{10}{0}\selectfont] (red_caption) {Common};
    \node[draw=blue!60, fill=blue!5] [below=0.2cm of red] (blue) {};
    \node [right=0.1cm of blue, font=\fontsize{10}{0}\selectfont] (blue_caption) {Shared};
    \node[draw=green!60, fill=green!5] [below=0.2cm of blue] (green) {};
    \node [right=0.1cm of green, font=\fontsize{10}{0}\selectfont] (green) {Task-specific};
    
    % IMAGE BATCH
    \node[imagenode] [below=1cm of conv_1_A] (image_A_1) {};
    \node[imagenode] [below=0.9cm of conv_1_A] (image_A_2) {};
    \node[imagenode] [below=0.8cm of conv_1_A] (image_A_3) {};
    \node[imagenode] [below=0.7cm of conv_1_A] (image_A_4) {};
    
    \node[] [below=-0.15cm of conv_1_A] (arrow_anchor_A_north) {};
    \node[] [above=-0.1cm of image_A_4] (arrow_anchor_A_south) {};
    \draw[->, thick] (arrow_anchor_A_south) -- (arrow_anchor_A_north);
    \node[] [left=1cm of image_A_3, align=left] (images_label) {image\\batch};
    
    \node[imagenode] [below=1cm of conv_1_B] (image_B_1) {};
    \node[imagenode] [below=0.9cm of conv_1_B] (image_B_2) {};
    \node[imagenode] [below=0.8cm of conv_1_B] (image_B_3) {};
    \node[imagenode] [below=0.7cm of conv_1_B] (image_B_4) {};
    
    \node[] [below=-0.15cm of conv_1_B] (arrow_anchor_B_north) {};
    \node[] [above=-0.1cm of image_B_4] (arrow_anchor_B_south) {};
    \draw[->, thick] (arrow_anchor_B_south) -- (arrow_anchor_B_north);
    
    \node[imagenode] [below=1cm of conv_1_C] (image_C_1) {};
    \node[imagenode] [below=0.9cm of conv_1_C] (image_C_2) {};
    \node[imagenode] [below=0.8cm of conv_1_C] (image_C_3) {};
    \node[imagenode] [below=0.7cm of conv_1_C] (image_C_4) {};
    
    \node[] [below=-0.15cm of conv_1_C] (arrow_anchor_C_north) {};
    \node[] [above=-0.1cm of image_C_4] (arrow_anchor_C_south) {};
    \draw[->, thick] (arrow_anchor_C_south) -- (arrow_anchor_C_north);

    %--------------------------------------
    %Lines
    %--------------------------------------
    
    % NETWORK A (One task)
    \draw[-] (conv_1_A) -- (conv_2_A);
    \draw[-] (conv_2_A) -- (conv_3_A);
    \draw[-] (conv_3_A) -- (conv_4_A);
    \draw[-] (conv_4_A) -- (conv_5_A);
    \draw[-] (conv_5_A) -- (conv_6_A);
    \draw[-] (conv_6_A) -- (conv_7_A);
    
    % single node
    \draw[dashed] (lower_left) -- (lower_right);
    \draw[dashed] (lower_left) -- (upper_left);
    \draw[dashed] (upper_left) -- (upper_right);
    \draw[dashed] (upper_right) -- (lower_right);

    % NETWORK B
    \draw[-] (conv_1_B) -- (conv_2_B);
    \draw[-] (conv_2_B) -- (conv_3_B);
    \draw[-] (conv_3_B.north) -- (conv_4_B.south);
    \draw[-] (conv_4_B.north) -- (conv_5_B.south);
    \draw[-] (conv_5_B) -- (conv_6_B);
    \draw[-] (conv_6_B) -- (conv_7_B);
    \draw[-] (conv_4_B.north) -- (conv_8_B.south);
    \draw[-] (conv_8_B) -- (conv_9_B);
    \draw[-] (conv_9_B) -- (conv_10_B);
    \draw[-] (conv_10_B) -- (conv_11_B);
    
    % NETWORK C
    \draw[-] (conv_1_C) -- (conv_2_C);
    \draw[-] (conv_2_C) -- (conv_3_C);
    \draw[-] (conv_3_C.north) -- (conv_4_C.south);
    \draw[-] (conv_4_C.north) -- (conv_5_C.south);
    \draw[-] (conv_5_C) -- (conv_6_C);
    \draw[-] (conv_6_C) -- (conv_7_C);
    \draw[-] (conv_4_C.north) -- (conv_8_C.south);
    \draw[-] (conv_8_C) -- (conv_9_C);
    \draw[-] (conv_9_C) -- (conv_10_C);
    \draw[-] (conv_10_C) -- (conv_11_C);
    \draw[-] (conv_3_C.north) -- (conv_12_C.south);
    \draw[-] (conv_12_C) -- (conv_13_C);
    \draw[-] (conv_13_C) -- (conv_14_C);
    \draw[-] (conv_14_C) -- (conv_15_C);

\end{tikzpicture}

==> tables/main_experiments_cifar.tex <==
\begin{tabular}{c|cc}
    \hline
    \multicolumn{3}{c}{\textbf{w/o pretraining}} \\
    \hline
    \textbf{Method} & \textbf{Acc} & \textbf{FM} \\
    \hline
Upperbound                                       & 0.8467±0.0143 & 0.0183±0.005  \\
EWC \cite{DBLP:journals/corr/KirkpatrickPRVD16}  & 0.5963±0.016  & 0.12±0.0166   \\
ER \cite{DBLP:journals/corr/abs-1902-10486}      & 0.7522±0.0219 & 0.0884±0.0142 \\
A-GEM \cite{DBLP:journals/corr/abs-1812-00420}   & 0.503±0.0495  & 0.3297±0.054  \\
PNN \cite{DBLP:journals/corr/RusuRDSKKPH16}     & \textbf{0.7838±0.0137} & \textbf{0.0±0.0} \\
LWF \cite{DBLP:journals/corr/LiH16e}             & 0.3666±0.0459 & 0.4619±0.0429 \\
HAT \cite{DBLP:journals/corr/abs-1801-01423}    & 0.748±0.0137  & 0.0001±0.0001 \\
CAT \cite{10.5555/3495724.3497277} & 0.6994±0.0072 & 0.0801±0.0151 \\
Ours                                            & 0.73±0.0137   & \textbf{0.0±0.0} \\



\hline
\multicolumn{3}{c}{\textbf{w/ pretraining}} \\
\hline
\textbf{Method} & \textbf{Acc} & \textbf{FM} \\
\hline
Upperbound                                       & 0.8702±0.0125 & 0.0137±0.0018 \\
EWC \cite{DBLP:journals/corr/KirkpatrickPRVD16}  & 0.6543±0.0226 & 0.1921±0.0205 \\
ER \cite{DBLP:journals/corr/abs-1902-10486}      & \textbf{0.8152±0.0146} & 0.0555±0.0079 \\
A-GEM \cite{DBLP:journals/corr/abs-1812-00420}   & 0.5227±0.0471 & 0.3411±0.0456 \\
LWF \cite{DBLP:journals/corr/LiH16e}             & 0.5379±0.0374 & 0.2992±0.025  \\
Ours                                            & 0.8091±0.0102 & \textbf{0.0±0.0} \\
    \hline
\end{tabular}

==> tables/main_experiments_core.tex <==
\begin{tabular}{c|cc}
    \hline
    \multicolumn{3}{c}{\textbf{w/o pretraining}} \\
    \hline
    \textbf{Method} & \textbf{Acc} & \textbf{FM} \\
    \hline
Upperbound                                      & 0.9957±0.0025 & 0.0031±0.0025  \\
EWC \cite{DBLP:journals/corr/KirkpatrickPRVD16} & 0.6325±0.0469 & 0.3663±0.0475   \\
ER \cite{DBLP:journals/corr/abs-1902-10486}     & 0.8848±0.0238 & 0.1143±0.024 \\
A-GEM \cite{DBLP:journals/corr/abs-1812-00420}  & 0.6567±0.0339 & 0.339±0.033  \\
PNN \cite{DBLP:journals/corr/RusuRDSKKPH16}     & \textbf{0.9986±0.0005} & \textbf{0.0±0.0} \\
LWF \cite{DBLP:journals/corr/LiH16e}            & 0.5035±0.0385 & 0.4963±0.0386 \\
HAT \cite{DBLP:journals/corr/abs-1801-01423}    & 0.8393±0.3197 & 0.0001±0.0001 \\
CAT \cite{10.5555/3495724.3497277} & 0.9932±0.0012  & 0.003±0.001 \\
Ours                                            & 0.9955±0.002           & \textbf{0.0±0.0} \\



\hline
\multicolumn{3}{c}{\textbf{w/ pretraining}} \\
\hline
\textbf{Method} & \textbf{Acc} & \textbf{FM} \\
\hline
Upperbound                                      & 0.996±0.0033  & 0.0034±0.0033 \\
EWC \cite{DBLP:journals/corr/KirkpatrickPRVD16} & 0.8082±0.0556 & 0.171±0.0655 \\
ER \cite{DBLP:journals/corr/abs-1902-10486}     & 0.895±0.022   & 0.1004±0.0213 \\
A-GEM \cite{DBLP:journals/corr/abs-1812-00420}  & 0.6383±0.0406 & 0.3289±0.0427 \\
LWF \cite{DBLP:journals/corr/LiH16e}            & 0.5571±0.0562 & 0.4412±0.0561  \\
Ours                                            & \textbf{0.9955±0.002}  & \textbf{0.0±0.0} \\
    \hline
\end{tabular}

==> tables/main_experiments_tinyimagenet.tex <==
\begin{tabular}{c|cc}
    \hline
    \multicolumn{3}{c}{\textbf{w/o pretraining}} \\
    \hline
    \textbf{Method} & \textbf{Acc} & \textbf{FM} \\
    \hline
Upperbound                                      &  0.5289±0.0212 & 0.0831±0.0165  \\
EWC \cite{DBLP:journals/corr/KirkpatrickPRVD16} &  0.4324±0.0111 & 0.0318±0.0029   \\
ER \cite{DBLP:journals/corr/abs-1902-10486}     &  0.5219±0.0075 & 0.1265±0.0097 \\
A-GEM \cite{DBLP:journals/corr/abs-1812-00420}  &  0.349±0.0617  & 0.3036±0.0609  \\
PNN \cite{DBLP:journals/corr/RusuRDSKKPH16}     & \textbf{0.5577±0.0054} & \textbf{0.0±0.0} \\
LWF \cite{DBLP:journals/corr/LiH16e}            &  0.2844±0.0194 & 0.352±0.0145 \\
HAT \cite{DBLP:journals/corr/abs-1801-01423}    & 0.53±0.0071 & 0.0001±0.0001 \\
CAT \cite{10.5555/3495724.3497277} & 0.4567±0.0051 & 0.0597±0.0147 \\
Ours                                            & 0.5218±0.0074 & \textbf{0.0±0.0} \\



\hline
\multicolumn{3}{c}{\textbf{w/ pretraining}} \\
\hline
\textbf{Method} & \textbf{Acc} & \textbf{FM} \\
\hline
Upperbound                                      &  0.7±0.0034    & 0.012±0.0021 \\
EWC \cite{DBLP:journals/corr/KirkpatrickPRVD16} &  0.5399±0.017  & 0.0899±0.0079 \\
ER \cite{DBLP:journals/corr/abs-1902-10486}     &  0.5735±0.0143 & 0.1197±0.0114 \\
A-GEM \cite{DBLP:journals/corr/abs-1812-00420}  &  0.4208±0.0174 & 0.2699±0.0202 \\
LWF \cite{DBLP:journals/corr/LiH16e}            &  0.3983±0.0076 & 0.3141±0.0065  \\
Ours                                            & \textbf{0.5811±0.005}  & \textbf{0.0±0.0} \\
    \hline
\end{tabular}

==> tables/main_results.tex <==
\begin{tabular}{c|cccccc}
        \hline
        \multicolumn{7}{c}{\textbf{w/o pretraining}} \\
        \hline
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Split Cifar}} & \multicolumn{2}{c}{\textbf{Split Tiny ImageNet}} & \multicolumn{2}{c}{\textbf{CORe50}}  \\
         \cline{2-7}
        & \textbf{Acc} & \textbf{FM} & \textbf{Acc} & \textbf{FM} & \textbf{Acc} & \textbf{FM} \\
        \hline
 Upperbound                                      &  0.8467±0.0143 & 0.0183±0.005  & 0.5289±0.0212 & 0.0831±0.0165   & 0.9957±0.0025 & 0.0031±0.0025 \\
 EWC \cite{DBLP:journals/corr/KirkpatrickPRVD16} &  0.5963±0.016  & 0.12±0.0166   & 0.4324±0.0111 & 0.0318±0.0029 & 0.6325±0.0469 & 0.3663±0.0475 \\
 ER \cite{DBLP:journals/corr/abs-1902-10486}     &  0.7522±0.0219 & 0.0884±0.0142 & 0.5219±0.0075 & 0.1265±0.0097 & 0.8848±0.0238 & 0.1143±0.024  \\
 A-GEM \cite{DBLP:journals/corr/abs-1812-00420}  &  0.503±0.0495  & 0.3297±0.054  & 0.349±0.0617  & 0.3036±0.0609 & 0.6567±0.0339 & 0.339±0.033   \\
 PNN \cite{DBLP:journals/corr/RusuRDSKKPH16}     & \textbf{0.7838±0.0137} & \textbf{0.0±0.0}       & \textbf{0.5577±0.0054} & \textbf{0.0±0.0}       & \textbf{0.9986±0.0005} & \textbf{0.0±0.0}       \\
 LWF \cite{DBLP:journals/corr/LiH16e}            &  0.3666±0.0459 & 0.4619±0.0429 & 0.2844±0.0194 & 0.352±0.0145  & 0.5035±0.0385 & 0.4963±0.0386 \\
 HAT \cite{DBLP:journals/corr/abs-1801-01423}    & 0.748±0.0137  & 0.0001±0.0001 & 0.53±0.0071 & 0.0001±0.0001 & 0.8393±0.3197 & 0.0001±0.0001   \\
 CAT \cite{10.5555/3495724.3497277} & 0.6994±0.0072 & 0.0801±0.0151 & 0.4567±0.0051 & 0.0597±0.0147 & 0.9932±0.0012  & 0.003±0.001 \\
 Ours                                            & 0.73±0.0137   & \textbf{0.0±0.0}       & 0.5218±0.0074 & \textbf{0.0±0.0}       & 0.9955±0.002           & \textbf{0.0±0.0}           \\



\hline
\multicolumn{7}{c}{\textbf{w/ pretraining}} \\
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Split Cifar}} & \multicolumn{2}{c}{\textbf{Split Tiny ImageNet}} & \multicolumn{2}{c}{\textbf{CORe50}}  \\
         \cline{2-7}
        & \textbf{Acc} & \textbf{FM} & \textbf{Acc} & \textbf{FM} & \textbf{Acc} & \textbf{FM} \\
\hline
 Upperbound                                      &  0.8702±0.0125 & 0.0137±0.0018 & 0.7±0.0034    & 0.012±0.0021  & 0.996±0.0033  & 0.0034±0.0033 \\
 EWC \cite{DBLP:journals/corr/KirkpatrickPRVD16} &  0.6543±0.0226 & 0.1921±0.0205 & 0.5399±0.017  & 0.0899±0.0079 & 0.8082±0.0556 & 0.171±0.0655  \\
 ER \cite{DBLP:journals/corr/abs-1902-10486}     &  \textbf{0.8152±0.0146} & 0.0555±0.0079 & 0.5735±0.0143 & 0.1197±0.0114 & 0.895±0.022   & 0.1004±0.0213 \\
 A-GEM \cite{DBLP:journals/corr/abs-1812-00420}  &  0.5227±0.0471 & 0.3411±0.0456 & 0.4208±0.0174 & 0.2699±0.0202 & 0.6383±0.0406 & 0.3289±0.0427 \\
 LWF \cite{DBLP:journals/corr/LiH16e}            &  0.5379±0.0374 & 0.2992±0.025  & 0.3983±0.0076 & 0.3141±0.0065 & 0.5571±0.0562 & 0.4412±0.0561 \\
 Ours                                            & 0.8091±0.0102 & \textbf{0.0±0.0}       & \textbf{0.5811±0.005}  & \textbf{0.0±0.0}       & \textbf{0.9955±0.002}  & \textbf{0.0±0.0}       \\
        \hline
        \end{tabular}

==> tables/parameters.tex <==
\begin{tabular}{c|c}
    \hline
    \textbf{Method} & \textbf{\#parameters} \\
    \hline
Upperbound                                      &           11M \\
EWC \cite{DBLP:journals/corr/KirkpatrickPRVD16} &           11M \\
ER \cite{DBLP:journals/corr/abs-1902-10486}     &           11M \\
A-GEM \cite{DBLP:journals/corr/abs-1812-00420}  &           11M \\
PNN \cite{DBLP:journals/corr/RusuRDSKKPH16}     &           39M \\
LWF \cite{DBLP:journals/corr/LiH16e}            &           11M \\
HAT \cite{DBLP:journals/corr/abs-1801-01423}    &           28M \\
CAT \cite{10.5555/3495724.3497277} & 90M \\
Ours                                            &           193M \\
\hline
\end{tabular}
